A Duality as a Theory for the Electroweak Interactions

We present a model based on a SU(2) confining theory which is dual to the standard model. This duality allows to calculate the electroweak mixing angle and the Higgs boson mass. Possible tests of this duality are discussed.

==> misc/Bmass <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
5 1 0 2 0 7 50 0 -1 0.000 0 1 0 0 1260.000 1530.000 990 1530 1260 1800 1530 1530
5 1 0 2 0 7 50 0 -1 0.000 0 0 0 0 1260.000 1530.000 990 1530 1260 1260 1530 1530
1 2 1 2 0 7 50 0 -1 4.000 1 0.0000 1260 540 270 270 990 540 1530 540
2 1 1 2 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 540 810 2070 810
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 540 1530 1080 1530
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 1530 1530 2070 1530
4 0 0 50 0 0 12 0.0000 4 135 135 810 1440 Y\001
4 0 0 50 0 0 12 0.0000 4 135 135 1575 1440 Y\001
4 0 0 50 0 32 12 0.0000 4 135 105 1215 990 l\001
4 0 0 50 0 0 12 0.0000 4 75 105 1215 1170 +\001


==> misc/Bmass2 <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
5 1 0 2 0 7 50 0 -1 0.000 0 1 0 0 3105.000 810.000 2835 810 3105 1080 3375 810
5 1 0 2 0 7 50 0 -1 0.000 0 0 0 0 3105.000 765.000 2835 765 3105 495 3375 765
1 2 1 2 0 7 50 0 -1 4.000 1 0.0000 1260 540 270 270 990 540 1530 540
2 1 1 2 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 540 810 2070 810
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 2385 810 2925 810
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 3375 810 3915 810
4 0 0 50 0 32 12 0.0000 4 135 105 1215 990 l\001
4 0 0 50 0 0 12 0.0000 4 75 105 2160 855 +\001
4 0 0 50 0 0 12 0.0000 4 135 135 3465 720 Y\001
4 0 0 50 0 0 12 0.0000 4 135 135 2610 720 Y\001


==> misc/Fmass <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
5 1 1 2 0 7 50 0 -1 4.000 0 0 0 0 1350.000 1710.000 1080 1710 1350 1440 1620 1710
5 1 0 2 0 7 50 0 -1 0.000 0 1 0 0 1350.000 1710.000 1080 1710 1350 1980 1620 1710
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1620 1710 2160 1710
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1305 1890 1395 2070
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1395 1890 1305 2070
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 540 1710 1080 1710
4 0 0 50 0 0 12 0.0000 4 135 135 945 1575 Y\001
4 0 0 50 0 0 12 0.0000 4 90 135 1260 2250 m\001
4 0 0 50 0 0 12 0.0000 4 135 60 1395 2340 f\001


==> misc/corrmass <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
5 1 0 2 0 7 50 0 -1 0.000 0 1 0 0 3105.000 810.000 2835 810 3105 1080 3375 810
5 1 0 2 0 7 50 0 -1 0.000 0 0 0 0 3105.000 765.000 2835 765 3105 495 3375 765
5 1 0 2 0 7 50 0 -1 0.000 0 1 0 0 -990.000 810.000 -1260 810 -990 1080 -720 810
5 1 1 2 0 7 50 0 -1 6.000 0 0 0 0 -990.000 765.000 -1260 765 -990 495 -720 765
1 2 1 2 0 7 50 0 -1 4.000 1 0.0000 1260 540 270 270 990 540 1530 540
2 1 1 2 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 540 810 2070 810
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 2385 810 2925 810
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 3375 810 3915 810
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1800 810 -1260 810
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -675 810 -135 810
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -945 990 -1035 1170
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1035 990 -945 1170
4 0 0 50 0 0 12 0.0000 4 75 105 2160 855 +\001
4 0 0 50 0 32 12 0.0000 4 135 105 1215 990 l\001
4 0 0 50 0 32 12 0.0000 4 135 105 3060 405 c\001
4 0 0 50 0 0 12 0.0000 4 135 135 1215 225 A\001
4 0 0 50 0 0 12 0.0000 4 135 135 2385 765 A\001
4 0 0 50 0 0 12 0.0000 4 135 135 3690 765 A\001
4 0 0 50 0 32 12 0.0000 4 135 105 3060 1215 c\001
4 0 0 50 0 0 12 0.0000 4 135 135 585 765 A\001
4 0 0 50 0 0 12 0.0000 4 135 135 2655 720 Y\001
4 0 0 50 0 0 12 0.0000 4 135 135 3420 720 Y\001
4 0 0 50 0 0 12 0.0000 4 135 135 1890 765 A\001
4 0 0 50 0 0 11 0.0000 4 105 1800 1350 1575 corrections to the boson mass\001
4 0 0 50 0 32 12 0.0000 4 135 105 -1755 720 c\001
4 0 0 50 0 0 12 0.0000 4 135 135 -1395 720 Y\001
4 0 0 50 0 0 12 0.0000 4 90 135 -1080 1305 m\001
4 0 0 50 0 0 12 0.0000 4 135 60 -945 1395 f\001
4 0 0 50 0 0 12 0.0000 4 135 135 -1080 450 A\001
4 0 0 50 0 32 12 0.0000 4 135 105 -270 720 c\001
4 0 0 50 0 0 11 0.0000 4 105 1875 -1980 1575 correction to the fermion mass\001


==> misc/shrockdiag <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
1 4 0 3 0 7 50 0 -1 0.000 1 0.0000 2137 720 26 26 2111 720 2163 720
1 4 0 3 0 7 50 0 -1 0.000 1 0.0000 2179 720 26 26 2153 720 2205 720
1 4 0 3 0 7 50 0 -1 0.000 1 0.0000 2115 1125 26 26 2089 1125 2141 1125
1 4 0 3 0 7 50 0 -1 0.000 1 0.0000 2070 1125 26 26 2044 1125 2096 1125
2 1 0 3 0 7 50 0 -1 0.000 0 0 -1 0 0 15
	 2250 2475 2250 6975 6750 6975 6975 6750 7200 7200 7425 6975
	 7425 6975 8550 6975 8550 1125 2250 1125 2250 1575 2025 1800
	 2475 2025 2250 2250 2250 2475
2 1 0 3 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5130 2475 5220 2475
2 1 0 3 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2655 5895 2745 5895
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3285 5895 3150 6075
2 5 0 1 0 -1 50 0 -1 0.000 0 0 -1 0 0 5
	0 <empty>
	 2025 675 2025 810 2295 810 2295 675 2025 675
3 0 0 3 0 7 50 0 -1 0.000 0 0 0 2
	 2250 6975 2250 7200
	 0.000 0.000
3 0 0 3 0 7 50 0 -1 0.000 0 0 0 2
	 3825 6975 3825 7200
	 0.000 0.000
3 0 0 3 0 7 50 0 -1 0.000 0 0 0 2
	 5400 6975 5400 7200
	 0.000 0.000
3 0 0 3 0 7 50 0 -1 0.000 0 0 0 2
	 2025 6975 2250 6975
	 0.000 0.000
3 0 0 3 0 7 50 0 -1 0.000 0 0 0 2
	 2025 5850 2250 5850
	 0.000 0.000
3 0 0 3 0 7 50 0 -1 0.000 0 0 0 2
	 2025 4500 2250 4500
	 0.000 0.000
3 0 0 3 0 7 50 0 -1 0.000 0 0 0 2
	 2025 3150 2250 3150
	 0.000 0.000
3 2 0 3 0 7 50 0 -1 0.000 0 0 0 4
	 2250 3825 3285 5265 4455 6075 5535 6300
	 0.000 -1.000 -1.000 0.000
4 0 0 50 0 0 12 0.0000 4 135 90 3825 7425 1\001
4 0 0 50 0 0 12 0.0000 4 135 90 5400 7425 2\001
4 0 0 50 0 0 12 0.0000 4 135 90 1800 6975 0\001
4 0 0 50 0 0 12 0.0000 4 135 90 2250 7425 0\001
4 0 0 50 0 32 20 0.0000 4 255 885 4950 2655 <cc>=0\001
4 0 0 50 0 32 20 0.0000 4 255 885 2475 6075 <cc>=0\001
4 0 0 50 0 0 12 0.0000 4 135 90 1800 5850 1\001
4 0 0 50 0 0 12 0.0000 4 135 90 1800 4500 2\001
4 0 0 50 0 0 12 0.0000 4 135 90 1800 3195 3\001

